Photoproduction of Pseudoscalar Mesons from Nuclei

The subject of this doctoral study is the pseudoscalar meson photoproduction from nuclei. Two types of processes are investigated in this regard: coherent and quasifree processes. In the case of the coherent process, we study it for the photoproduction of pion and eta mesons. We place special emphasis on the various sources that put into question earlier nonrelativistic-impulse-approximation calculations. These include: final-state interactions, relativistic effects, off-shell ambiguities, and violations to the impulse approximation. By far the largest uncertainty emerges from the ambiguity in extending the many on-shell-equivalent representations of the elementary amplitude off the mass shell. In the case of the quasifree process, we study it for the photoproduction of the kaon meson. We compute the recoil polarization of the lambda-hyperon and the photon asymmetry as well as the differential cross section. By introducing the notion of a ``bound-nucleon propagator'' we exploit Feynman's trace techniques to develop closed-form, analytic expressions for all photoproduction observables. Our results indicate that polarization observables are sensitive only to the fundamental physics, making them ideal tools for the study of modifications to the elementary process in the nuclear medium.

==> Laithdefs.tex <==
%auto-ignore
\makeatletter
\def\pmb#1{\leavevmode\setbox0=\hbox{#1}%
\kern-.02em\copy0\kern-\wd0
\kern.04em\copy0\kern-\wd0
\kern-.02em\raise.04em\box0 }

%\usepackage{feynmf}
%\usepackage[dvips]{graphics}
%\usepackage{rotating}

\def\notA{{\hbox{$A$}\kern-5.87pt{/}\ }}
\def\notD{{\hbox{$D$}\kern-7.37pt{/}\ }}
\def\notcalD{{\hbox{${\cal D}$}\kern-6.87pt{/}\ }}
\def\notcalA{{\hbox{${\cal A}$}\kern-6.87pt{/}\ }}
\def\notp{{\hbox{$p$}\kern-5.87pt{/}\ }}
\def\notpartial{{\hbox{$\partial$}\kern-5.87pt{/}\ }}
\def\notDO{{\hbox{O}\kern-7.37pt{/}\ }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\entrylabel}[1]{\mbox{\textsf{#1:}}\hfil}
\newenvironment{entry}%
 {\begin{list}{}%
   {\renewcommand{\makelabel}{\entrylabel}%
    \setlength{\labelwidth}{3cm}%
    \setlength{\leftmargin}{1.25in}
%    \setlength{\rightmargin}{1in}
   }%
 }%
{\end{list}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% begin new commands from Joergen Beck Hanson
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\BEQN}     {\begin{eqnarray}}
\newcommand{\EEQN}     {\end{eqnarray}}
\newcommand{\BFIG}     {\begin{figure}\centering}
\newcommand{\EFIG}     {\end{figure}}
\newcommand{\BEQNA}    {\renewcommand{\arraystretch}{1.75}\begin{equation}\begin{array}{rcl}}
\newcommand{\EEQNA}    {\end{array}\end{equation}\renewcommand{\arraystretch}{1}}
\newcommand{\refmat}[1]   {equation~\ref{#1}}
\newcommand{\reffig}[1]   {figure~\ref{#1}}
\newcommand{\reftab}[1]   {table~\ref{#1}}
\newcommand{\mw}       {\mbox{$ {\mathrm M}_{\mathrm W}$}}
\newcommand{\gw}       {\mbox{$ \Gamma_{\mathrm W}$}}
\newcommand{\mz}       {\mbox{$ {\mathrm M}_{\mathrm Z}$}}
\newcommand{\mws}       {\mbox{$ {\mathrm M}_{\mathrm W}^2$}}
\newcommand{\mzs}       {\mbox{$ {\mathrm M}_{\mathrm Z}^2$}}
\newcommand{\mh}       {\mbox{$ {\mathrm M}_{\mathrm H}$}}
\newcommand{\mt}       {\mbox{$ {\mathrm M}_{\mathrm t}$}}
\newcommand{\w}        {\mbox{$ {\mathrm W}$}}
\newcommand{\Wp}       {\mbox{$ {\mathrm W}^+ $}}
\newcommand{\Wm}       {\mbox{$ {\mathrm W}^- $}}
\newcommand{\wpm}      {\mbox{$ {\mathrm W}^{\pm} $}}
\newcommand{\photon}   {\mbox{$ \gamma$}}
\newcommand{\A}        {\mbox{$ {\mathrm A}$}}
\newcommand{\z}        {\mbox{$ {\mathrm Z}^0$}}
\newcommand{\ee}       {\mbox{$ {\mathrm e}^+ {\mathrm e}^-$}}
\newcommand{\ww}       {\mbox{$ {\mathrm W}^+ {\mathrm W}^-$}}
\newcommand{\zz}       {\mbox{$ {\mathrm Z}^0 {\mathrm Z}^0$}}
\newcommand{\wz}       {\mbox{$ \z \w$}}
\newcommand{\wwz}      {\mbox{$ \z \ww$}}
\newcommand{\wwgamma}  {\mbox{$ \gamma \ww$}}
\newcommand{\eeff}     {\mbox{$ \ee \rightarrow {\mathrm f} \bar{{\mathrm f}}$}}
\newcommand{\eezgammaff}     {\mbox{$ \ee \rightarrow \z /\photon \rightarrow
    {\mathrm f} \bar{{\mathrm f}}$}}
\newcommand{\eeffff}   {\mbox{$ \ee \rightarrow {\mathrm f}_1 \bar{{\mathrm
        f}_2} {\mathrm f}_3 \bar{{\mathrm f}_4} $}}
\newcommand{\eewwffff} {\mbox{$ \ee \rightarrow \ww \rightarrow {\mathrm f}_1
    \bar{{\mathrm f}_2} {\mathrm f}_3 \bar{{\mathrm f}_4} $}}
\newcommand{\eeww}     {\mbox{$ \ee \rightarrow \ww$}}
\newcommand{\wwqqlv}   {\mbox{$ \ww \rightarrow qq \ell \nu $}}
\newcommand{\wwjjlv}   {\mbox{$ \ww \rightarrow jj \ell \nu $}}
\newcommand{\wwjjev}   {\mbox{$ \ww \rightarrow jj e \nu $}}
\newcommand{\wwjjmv}   {\mbox{$ \ww \rightarrow jj \mu \nu $}}
\newcommand{\wwjjjj}   {\mbox{$ \ww \rightarrow jjjj$}}
\newcommand{\lvlv}     {\mbox{$ \ell \nu \ell \nu$}}
\newcommand{\lvqq}     {\mbox{$ \ell \nu q \bar{q}$}}
\newcommand{\evqq}     {\mbox{$ e \nu q \bar{q}$}}
\newcommand{\muvqq}     {\mbox{$ \mu \nu q \bar{q}$}}
\newcommand{\lvjj}     {\mbox{$ \ell \nu j j$}}
\newcommand{\evjj}     {\mbox{$ e\nu jj$}}
\newcommand{\muvjj}     {\mbox{$ \mu\nu jj$}}
\newcommand{\jjev}     {\mbox{$jj e\nu$}}
\newcommand{\jjmv}     {\mbox{$jj\mu\nu$}}
\newcommand{\tauvjj}     {\mbox{$ \tau\nu jj$}}
\newcommand{\evev}     {\mbox{$ e\nu e\nu $}}
\newcommand{\evmuv}     {\mbox{$ e\nu \mu\nu $}}
\newcommand{\evtauv}     {\mbox{$ e\nu \tau\nu $}}
\newcommand{\muvmuv}     {\mbox{$ \mu\nu \mu\nu $}}
\newcommand{\muvtauv}     {\mbox{$ \mu\nu \tau\nu $}}
\newcommand{\tauvtauv}     {\mbox{$ \tau\nu \tau\nu $}}
\newcommand{\eeee}     {\mbox{$ \ee\ee$}}
\newcommand{\evud}     {\mbox{$ {\mathrm e}^- \bar{\nu}_e {\mathrm u}
    \bar{{\mathrm d}}$}}
\newcommand{\qqqq}     {\mbox{$ q q q q$}}
\newcommand{\jjjj}     {\mbox{$ j j j j$}}
\newcommand{\ppbar}    {\mbox{$ {\mathrm p} \bar{{\mathrm p}} $}}
\newcommand{\pantip}   {\mbox{$ {\mathrm p} \bar{{\mathrm p}} $}}
\newcommand{\gev}      {\mbox{GeV}}
\newcommand{\mev}      {\mbox{MeV}}
\newcommand{\tev}      {\mbox{TeV}}
\newcommand{\nb}       {\mbox{nb}}
\newcommand{\nbinv}    {\mbox{nb$^{-1}$}}
\newcommand{\pb}       {\mbox{pb}}
\newcommand{\pbinv}    {\mbox{pb$^{-1}$}}
\newcommand{\pantiptowgamma}      {\mbox{$ \pantip\rightarrow\w\gamma $}}
\newcommand{\lv}       {\mbox{$ \ell \nu$}}
\newcommand{\qqbar}    {\mbox{$ q \bar{q}$}}
\newcommand{\vt}       {\vartheta}
\newcommand{\kg}{\kappa_\gamma}
\newcommand{\kZ}{\kappa_Z}
\newcommand{\lmg}{\lambda_\gamma}
\newcommand{\lZ}{\lambda_Z}
\newcommand{\dZ}{\delta_Z}
\newcommand{\xg}{x_\gamma}
\newcommand{\xZ}{x_Z}
\newcommand{\yg}{y_\gamma}
\newcommand{\yZ}{y_Z}
\newcommand{\pvl}{{\vec p}_l}
\newcommand{\pvlb}{{\vec p}_{\bar{l}}}
\newcommand{\pvn}{{\vec p}_{\nu}}
\newcommand{\pvnb}{{\vec p}_{\bar{\nu}}}

%Standard journal references
\def\ap#1#2#3   {{\em Ann. Phys. (NY)} {\bf#1} (#2) #3.}
\def\apj#1#2#3  {{\em Astrophys. J.} {\bf#1} (#2) #3.}
\def\apjl#1#2#3 {{\em Astrophys. J. Lett.} {\bf#1} (#2) #3.}
\def\app#1#2#3  {{\em Acta. Phys. Pol.} {\bf#1} (#2) #3.}
\def\ar#1#2#3   {{\em Ann. Rev. Nucl. Part. Sci.} {\bf#1} (#2) #3.}
\def\cpc#1#2#3  {{\em Computer Phys. Comm.} {\bf#1} (#2) #3.}
\def\err#1#2#3  {{\it Erratum} {\bf#1} (#2) #3.}
\def\ib#1#2#3   {{\it ibid.} {\bf#1} (#2) #3.}
\def\jmp#1#2#3  {{\em J. Math. Phys.} {\bf#1} (#2) #3.}
\def\ijmp#1#2#3 {{\em Int. J. Mod. Phys.} {\bf#1} (#2) #3.}
\def\jetp#1#2#3 {{\em JETP Lett.} {\bf#1} (#2) #3.}
\def\jpg#1#2#3  {{\em J. Phys. G.} {\bf#1} (#2) #3.}
\def\mpl#1#2#3  {{\em Mod. Phys. Lett.} {\bf#1} (#2) #3.}
\def\nat#1#2#3  {{\em Nature (London)} {\bf#1} (#2) #3.}
\def\nc#1#2#3   {{\em Nuovo Cim.} {\bf#1} (#2) #3.}
\def\nim#1#2#3  {{\em Nucl. Instr. Meth.} {\bf#1} (#2) #3.}
\def\np#1#2#3   {{\em Nucl. Phys.} {\bf#1} (#2) #3.}
\def\pcps#1#2#3 {{\em Proc. Cam. Phil. Soc.} {\bf#1} (#2) #3.}
\def\pl#1#2#3   {{\em Phys. Lett.} {\bf#1} (#2) #3.}
\def\prep#1#2#3 {{\em Phys. Rep.} {\bf#1} (#2) #3.}
\def\prev#1#2#3 {{\em Phys. Rev.} {\bf#1} (#2) #3.}
\def\prl#1#2#3  {{\em Phys. Rev. Lett.} {\bf#1} (#2) #3.}
\def\prs#1#2#3  {{\em Proc. Roy. Soc.} {\bf#1} (#2) #3.}
\def\ptp#1#2#3  {{\em Prog. Th. Phys.} {\bf#1} (#2) #3.}
\def\ps#1#2#3   {{\em Physica Scripta} {\bf#1} (#2) #3.}
\def\rmp#1#2#3  {{\em Rev. Mod. Phys.} {\bf#1} (#2) #3.}
\def\rpp#1#2#3  {{\em Rep. Prog. Phys.} {\bf#1} (#2) #3.}
\def\sjnp#1#2#3 {{\em Sov. J. Nucl. Phys.} {\bf#1} (#2) #3.}
\def\spj#1#2#3  {{\em Sov. Phys. JEPT} {\bf#1} (#2) #3.}
\def\spu#1#2#3  {{\em Sov. Phys.-Usp.} {\bf#1} (#2) #3.}
\def\zp#1#2#3   {{\em Zeit. Phys.} {\bf#1} (#2) #3.}

\newcommand{\putpicture}[3]{%
\IfFileExists{#3}{\resizebox{#1}{#2}{\includegraphics{#3}}}
 {\resizebox{#1}{#2}{File
   #3 \\ is missing}}
}
\newcommand{\putpic}[1]{
  \IfFileExists{#1}{\includegraphics{#1}}
 {\resizebox{5cm}{5cm}{File
   #1 \\ is missing}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% end from Joergen Beck Hanson
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\makeatother

\widowpenalty=10000
\clubpenalty=10000
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.5}
\renewcommand{\floatpagefraction}{0.8}
\renewcommand{\textfraction}{0.1}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}
\pretolerance=500
\tolerance=1000 
\hbadness=3000
\vbadness=3000
\hyphenpenalty=400

%%%  some struts for tables  (mimi)
\newcommand{\strutrule}{\vrule height16pt width0pt depth9pt}
\newcommand{\ruleup}{\vrule height16pt width0pt depth0pt}
\newcommand{\bigruleup}{\vrule height20pt width0pt depth0pt}
\newcommand{\ruledown}{\vrule height0pt width0pt depth10pt}
\newcommand{\bigruledown}{\vrule height0pt width0pt depth20pt}


\endinput

==> NuclearStructureold.tex <==
%auto-ignore
\chapter{Relativistic Nuclear Structure}
\label{ch:NuclearStructure}


Relativistic nuclear structure formalisms represent a growing field of
study where the nuclear structure is determined using fully
relativistic models. It has been argued for a long time that due to
the relative small binding of the nucleons in nuclei, nonrelativistic
formalisms should be adequate to describe the nuclear structure. This
assertion is impressively challenged in the relativistic treatments,
where it has been suggested that the small binding energy is a result
of a cancellation between two large potentials with different Lorentz
transformation properties, with one of the potentials being attractive
and the other repulsive.


Not only that the relativistic formalisms point to the importance of
relativistic effects, but it also provide us
with a more credible and aesthetic theory. This is because the
relativistic formalism is an effective field theory as opposed to the
``ad hoc'' potential-based nonrelativistic formalisms. Thus the theory is
physical and consistent with quantum-field-theory
principles. Furthermore, aspects of the nuclear force that has been
always put in the nonrelativistic formalisms by hand and with no
basis, appears naturally and with no effort in the relativistic
formalisms. Examples of these include spin-orbit coupling and
three-body forces.


Relativistic treatments have enjoyed a great success in recent years in
their description of the nuclear structure. They do have a number of
pitfalls that are systematically being surmounted and resolved. The
bottom line, however, lies in the experimental verification of these
formalisms. To this end, there is a well-planned experimental work
that may decisively proves the validity and applicability of these
formalisms.


\section{Quantum Hadrodynamics}

Quantum hadrodynamics (QHD) is a model for the study of the
relativistic nuclear many-body problem through an effective Lagrangian
field theory. The model was introduced by J. D. Walecka in
1974~\cite{serwal86}. It describes nuclear matter as resulting from
interactions between nucleons (baryons) in the nucleus through the
exchange of neutral scalar $\sigma$ and vector $\omega$
mesons. The couplings of these mesons to the baryon fields is achieved
by the minimal substitution as can be seen in Table \ref{QHD-I
parameters}. In this table, $g_s$ is the scalar coupling constant and $
g _v $ is the vector coupling constant. The model suggests a
nucleon-nucleon force which is attractive at large separations and
repulsive at short ones.
%%%
\begin{table}
\caption{The fields in quantum hadrodynamics.}
\vspace{.5cm}
\begin{center}
\thicklines
\begin {tabular} { clccc }
\hline
\hline
\thinlines
Field & Description & Particle & Mass & Coupling \\
\hline
\thicklines
$ \psi $ & Baryon & p, n,... & $M$ & \\ $ \phi $ & Neutral scalar
meson & $ \sigma $ & $ m _s $ & $ g _s \bar \psi \phi \psi $\\ $ V
_\mu $ & Neutral vector meson & $ \omega $ & $ m _v $ & $ g _v \bar
\psi \gamma ^ \mu V_\mu \psi $ \\
\hline
\hline
\end{tabular}
\end{center}
\label{QHD-I parameters}
\end{table}
%%
The Lagrangian for this system is as following:
%%%
\begin{equation}
{\cal L} = {\bar \psi} [ \gamma _ \mu ( i \partial ^ \mu - g_v V^ \mu)
- (M - g _s \phi ) ] \psi + \frac {1} {2} (\partial _ \mu \phi
\partial ^ \mu \phi - m _s ^2 \phi ^2) - \frac {1}{4} F_{\mu \nu}
F^{\mu \nu} + \frac {1} {2} m_v ^2 V_ \mu V^ \mu\,,
\end{equation}
%%%
where
%%%
\begin{equation}
F_{\mu \nu} \equiv \partial_\mu V_\nu - \partial _\nu V_\mu\,.
\end{equation}
%%%

The field equations can be derived then from the Lagrangian and one
obtains
%%%
\begin{equation}
(\partial_\mu \partial^\mu + {m_s}^2)\phi = g_s {\bar\psi} \psi\,,
\label{scalarequation}
\end{equation}
%%%
\begin{equation}
(\partial_\mu \partial^\mu + {m_v}^2) V^\nu= g_v {\bar\psi} \gamma^\nu
\psi\,,
\label{vectorequation}
\end{equation}
%%%
\begin{equation}
[\gamma _\mu(i\partial ^\mu - g_v V^\mu) - ( M - g _s \phi)] \psi =
0\,.
\label{nucleonequation}
\end{equation}
%%%
Hence we have a system of three coupled nonlinear differential
equations. Since solving these equations exactly is a formidable task,
one resorts to approximations like the mean-field picture known also
as the Hartree approximation. In this picture, the scalar and vector
fields are treated as classical fields, and one solve this system by
finding the configuration of these fields that solves all three
equations simultaneously. That is one finds a self-consistent solution
for this system. As a result, the nucleon equation
\ref{nucleonequation} becomes a one-body Dirac equation with a scalar
$g_s \phi$ and a vector $ g_v V^\mu$ potentials. One also finds that
the spatial components of the vector field have a vanishing
contribution in the static limit as a result of current
conservation. This is because we are restricting our discussion to
spherically symmetric nuclei with a total angular momentum of
zero. The mean-field equation then reads as
%%%
\begin{equation}
[i \gamma ^ \mu \partial _ \mu - g_v \gamma ^ 0 V({\mathbf x} ) - ( M - g
_s \phi ( {\mathbf x}) ) ] \psi = 0\,.
\end{equation}
%%%
The theory has three free parameters to be determined: $\{g_s,
g_v,m_s\}$. These are resolved using basic properties of
finite nuclei and infinite matter like the saturation density and the rms
charge radius of $^{40}$Ca.


In using the QHD model (known also as Walecka model) one finds that it
can successfully explain and predict many physical features of nuclei
with impressively a minimal number of phenomenological parameters that
are determined from only bulk properties of nuclei. The relativistic
structure is a keystone of this model. There are many consequences of
this relativistic treatment~\cite{serwal86}. One of them is the
existence of a nuclear shell model with the experimentally observed
level orderings, spacings, and major shell closures in nuclei.


Another consequence is the saturation of nuclear matter. This
saturation explains the stability of only a limited number of nuclei
which is what is observed in nature. The relatively small nuclear
binding energy of saturation is the result of a very delicate and fine
cancellation between a large scalar attraction and a large vector
repulsion.


A third consequence of the relativistic structure is the spin-orbit
splitting. The splitting here appears naturally and within the
structure of the theory unlike the nonrelativistic treatments. In
fact, we find a large spin-orbit splitting in this model as is
experimentally verified.


A final consequence of this model is the density dependence of the
interaction as the vector and scalar potentials have different density
dependence. This difference is the reason for the nuclear saturation
in this model. In the nonrelativistic treatments the density
dependence must be included phenomenologically.


The natural remarkable consequences of the QHD Hartree model testify
to its physical validity and to the ``smartness'' of Dirac equation
which within its simple but illusive structure can produce many
physical effects that are never dreamed of in the nonrelativistic
treatments.
	 

\section{Extensions to Quantum Hadrodynamics}

Since Walecka introduced the QHD model many extensions have been
achieved to improve its predictions. As a result, the original QHD
model presented above is now labeled as QHD-I. One extension is the
QHD-II introduced by Serot~\cite{serwal86} that incorporates charged
vector ${\rho}$ and charged pseudoscalar ${\pi}$ mesons in
addition to the $\sigma$ and $\omega$ mesons. The model also
incorporates the electromagnetic interaction through the photon field
$A^\mu$ to account for the Coulomb repulsion between protons in
nuclei. Table \ref{QHD-II parameters} lists the ingredients of this
model.
%%%%
\begin{table}
\caption{The fields in QHD-II.}
\vspace{.5cm}
\begin{center}
\thicklines
\begin {tabular} { clccc }
\hline
\hline
\thinlines
Field & Description & Particle & Mass & Coupling \\
\hline
\thicklines
$ \psi $ & Baryon & p, n,... & $M$ & \\

$ \phi $ & Neutral scalar meson & $ \sigma $ & $ m _s $ & $ g _s \bar
\psi \phi \psi $\\ 

$ V_\mu $ & Neutral vector meson & $ \omega $ & $ m _v $ & $ g _v \bar
\psi \gamma ^ \mu V_\mu \psi $ \\

\boldmath${\pi}$ \unboldmath& Charged pseudoscalar meson & $ \pi $ & $ m _\pi
$ & $ ig _\pi \bar \psi \gamma ^5
\mbox{\boldmath$\tau\cdot{\pi}$\unboldmath} \psi $ \\

$ {\mathbf b_\mu} $ & Charged vector meson & $ \rho $ & $ m _\rho $ &
$ \frac {1}{2} g_\rho \bar \psi \gamma^\mu$
\boldmath$\tau\cdot{b_\mu}$\unboldmath $\psi$ \\

$ {A_\mu} $ & Photon & $ \gamma $ & $ m_\gamma = 0$ & $ e
\bar \psi \gamma^\mu \frac {1}{2}(1 + \tau_3) A_\mu \psi $ \\
\hline
\hline
\end{tabular}
\end{center}
\label{QHD-II parameters}
\end{table}
%%%%
Other extensions that incorporate nonlinear terms for the meson fields
have also been introduced. QHD theory with these extensions provide us
today with a very successful model for describing nuclear matter in an
impressively transparent formalism. For the sake of brevity I will not
elaborate on these extensions but it is appropriate to mention that I
use only two versions of the QHD theory throughout this work namely
QHD-I and QHD-II.

Finally, we have used a standard set
of parameters for the Walecka model: $g_{ s}^{2}=109.63$,
$g_{ v}^{2}=190.43$, $g_{\rho}^{2}=65.23$, $m_{ s}=520$~MeV,
$m_{ v}=783$~MeV, and $m_{\rho}=770$~MeV.



\section{Mean Field Approximation to ${}^4$He}

In our study of meson photoproduction processes we have used ${}^4$He
as a nuclear target. In doing so, we needed to have a reasonable
description of the nuclear structure of ${}^4$He. We determined this
structure using a mean-field approximation to the Walecka model.  Even
though the use this approximation to describe a nucleus as small as
${}^{4}$He should be suspect, we feel justified in adopting this
choice. The reason is that the photoproduction processes we studied
are sensitive to only the bulk properties of ${}^4$He --- which can be
constrained by experiment. Consequently, in order to reproduce the
experimental charge density of ${}^{4}$He, we have modified the mass
of the $\sigma$ meson to $m_{ s}=564$~MeV --- while maintaining
constant the ratio of $g_{ s}^{2}/m_{ s}^{2}$. Figure
\ref{fig:HeFormFact} shows the ${}^4$He form factor
%%%
\BFIG
\centerline{\psfig{figure=HeFormFact.pstex,height=6.0in,width=6.0in}}
\caption[${}^4$He form factor using mean-field approximation to
Walecka model] {The ${}^4$He form factor as
calculated using the original parameters of Walecka model (QHD-II),
and then using the modified ones to fit the experimental form factor.}
\label{fig:HeFormFact}
\end{figure}
%%
as a function of momentum transfer ($q \equiv |{\bf q}|$) as calculated using the original parameters of Walecka model (QHD-II),
and then using the modified ones, to fit the experimental form factor
(included also in the figure). It is remarkable that by a small change in
only one of the parameters, we can fit the experimental form factor
almost perfectly. To be noted here that the calculation using QHD-I
gives also identical results to the QHD-II ones.

The experimental form factor in Figure \ref{fig:HeFormFact} is produced
using a phenomenological fit to data over a
wide range of momentum transfers and is parameterized according to the
following equation~\cite{cek87,bentan90}:
\begin{equation}
F^{ch}_{exp} = F_o (q) f^{ch}_{p} (q)\;,
\end{equation}
where  
\begin{equation}
F_o(q) = F(q) F_{c.m.}(q)\;,
\end{equation}
and
\begin{equation}
F_{c.m.}(q) = {\rm exp}\left( R^2 q^2 / 6 A \right) \;,
\end{equation}
%%%
\begin{equation}
F(q) = - \frac{3 \pi b \left[ cos(qc) - \pi b\,sin(qc) \, coth(\pi b q)/c
\right]} {q c^2 sinh(\pi b q) [ 1 + \pi^2 b^2 / c^2] }\;.
\end{equation}
Here the parameters $b$, $c$, and $R$ are given in Table
\ref{Tab:formfactorpar} for the three nuclei: ${}^4$He, ${}^{12}$C, and
${}^{40}$Ca.
%%%%
\begin{table}
\caption{Parameters of the nuclear form factor for ${}^4$He, ${}^{12}$C, and
${}^{40}$Ca.}
\vspace{.5cm}
\begin{center}
\thicklines
\begin {tabular} { cccc }
\hline
\hline
\thinlines
 & $b$ (fm) & $c$ (fm) & $R$ (fm) \\
\hline
\thicklines
${}^4$He & 0.406 & 1.231 & 1.806 \\ 
${}^{12}$C & 0.478 & 2.220 & 2.462 \\ 
${}^{40}$Ca & 0.537 & 3.573 & 3.287\\
\hline
\hline
\end{tabular}
\end{center}
\label{Tab:formfactorpar}
\end{table}


\section{Bound Nucleon Wavefunction}

As evident in the previous sections, the QHD theory reduces to finding
a solution to the nucleon Dirac equation
\ref{nucleonequation} with scalar and vector potentials in such away
that this solution is also self-consistent with the field equations
\ref{scalarequation} and
\ref{vectorequation}. It is proper here to give a brief idea of
the solutions to the Dirac equation with scalar and vector fields.


Concentrating on spherically symmetric nuclei one finds that the
fields $\phi$ and $V^0$ must be spherically symmetric too. Hence, We
can rewrite equation \ref{nucleonequation} for certain energy
eigenvalue $E$ with the new definitions of $S(r) = g_s \phi (r)$ and
$V(r) = g_v V^0 (r)$ as
%%%
\begin{equation}
H \psi = E \psi\,,
\end{equation}
%%%
where
%%%
\begin{equation}
H = \mbox{\boldmath$\alpha \cdot p$\unboldmath} + \beta (\,M - S(r)\,) +
V(r)\,.
\end{equation}
%%%
In this equation
%%%
\begin{equation}
\alpha _i \equiv \gamma _0 \gamma _ i\,,
\end{equation}
%%%
and
%%%
\begin{equation}
\beta \equiv \gamma _0\,.
\end{equation} 
%%%

We can find a set of commuting operators that also commute with the
Hamiltonian ($H$) of this equation. Consequently, these operators
provide us with constants of the motion that can be used to
characterize the energy eigenfunctions. Examples of these operators
include ${\mathbf J^2}$ (total angular momentum squared), $J_z$ (z-axis
projection of the total angular momentum), and $ K$ ~\cite{sak73} an
operator that is defined as
%%%
\begin{equation}
K \equiv \beta (2 {{\mathbf S} \cdot {\mathbf J} } - \frac {1} {2} ) =
\beta ({2 {\mathbf S} \cdot {\mathbf L}}+ 1)\,.
\end{equation}
%%%
The operator $K$ determines in the nonrelativistic limit whether the
projection of the spin is parallel or anti-parallel to the total
angular momentum. The eigenvalues for those operators are $ j(j+1)$
for $ {\mathbf J^2} $, $m$ for $J_z$, and $ -\kappa$ for $ K$.


It can be shown that there is a relationship between $ \kappa $ and
$j$ which is
%%%
\begin{equation}
\kappa = \pm (j + \frac {1} {2} )\,.
\end{equation}
%%%
Hence $ \kappa $ is a nonzero integer which can be positive or
negative. The sign of $ \kappa $ determines whether the spin is
parallel (positive) or anti-parallel (negative) in the nonrelativistic
limit.


We can write the four-component eigenfunction $ \psi $ as a vector of
two-component spinors
%%% 
\begin{equation}
\psi = {\psi _A \choose \psi _B}\,.
\end{equation}
%%%
By this decomposition one can show that even though the four component
eigenfunction is not an eigenfunction of $ {\mathbf L^2} $, the
spinors $
\psi _A$ and $ \psi _B$ are separately eigenfunctions with eigenvalues
$ l_A(l_A + 1)$, and $ l_B(l_B + 1)$ respectively. It can be shown
also that these eigenvalues are related to $ \kappa $ and $j$ through
the equations
%%%
\begin{equation}
- \kappa = j(j+1) - l_A(l_A+1) + \frac {1} {4}\,,
\end{equation}
%%%
and
%%%
\begin{equation}
\kappa = j(j+1) - l_B(l_B+1) + \frac {1} {4}\,.
\end{equation}
%%%
As a result any energy eigenfunction can be uniquely characterized by
only $E$, $ \kappa $, and $m$.

	The above analysis enables us to write $\psi$ as
%%%
\begin{equation}
\psi = {\psi _A \choose \psi _B} =  {g_{E\kappa}(r) {y } {^{m} _{j l_A}}  \choose i f_{E\kappa}(r) {y } {^{m} _{j l_B}}}\,,
\end{equation}
%%%
where ${y } {^{m} _{j l}} $ are the normalized spin-angular functions
constructed by the addition of Pauli spinors to the spherical
harmonics of order $l$. The inclusion of $i$ with $f_{E\kappa}(r)$
is in order to make $f_{E\kappa}(r)$ and $g_{E\kappa}(r)$ real for
bound-state solutions. Substituting this result back into the Dirac
equation and performing some algebra, we arrive at the coupled
equations:
%%%
\begin{equation}
-\frac {df} {dr} - \frac {(1-\kappa) } {r} f(r) = (E - V(r) - M +
S(r)\,) g(r)\,,
\end{equation}
%%%
\begin{equation}
\frac {dg} {dr} + \frac {(1+\kappa) } {r} g(r) = (E - V(r) + M -
S(r)\,) f(r)\,.
\end{equation}
%%%
Now writing these equations in terms of
%%%
\begin{equation}
F(r) = r f(r)\,,
\end{equation}
%%%
\begin{equation}
G(r) = r g(r)\,,
\end{equation}
%%%
we have
%%%
\begin{equation}
 \frac {dF} {dr} - \frac {\kappa} {r} F(r) = - (E - V(r) - M + S(r)\,) G(r)\,,
\end{equation}
%%%
\begin{equation}
 \frac {dG} {dr} + \frac {\kappa} {r} G(r) = (E - V(r) + M - S(r)\,) F(r)\,.
\end{equation}
%%%
These are two coupled differential equations which can be solved
numerically by the Runge-Kutta method. It is worth noting that there
is an implicit symmetry in these equations as $ F
\rightarrow G$ and $ G \rightarrow F$ if $ E \rightarrow -E$, $ V(r)
\rightarrow -V(r)$, and $ \kappa \rightarrow -\kappa $.


\section{Nuclear Densities in the Relativistic Formalism}

Nuclear densities in the relativistic formalisms are a vivid example
of the richness of relativity. While we have essentially only one
ground state density in the nonrelativistic formalisms: the vector
(matter) density, the relativistic formalism provide us with the
possibility of having up to five different densities: vector (matter),
tensor, scalar, axial-vector, and pseudoscalar. This richness is a result of the fact that in the space of Dirac spinors
we can have up to 16 linearly-independent matrices. These
form the set: $\{1, \gamma ^\mu, \gamma ^\mu \gamma ^5, i \gamma ^5,
\sigma ^{\mu \nu} \}$ of bilinear covariants. The covariants transform
as 
scalar, vector, axial-vector, pseudoscalar, and tensor respectively
under Lorentz transformations (Poincar\'e group). It is important to
note that the densities are truly independent and constitute
fundamental nuclear-structure quantities. The fact that in the
nonrelativistic framework only one density survives is due to the
limitation of the approach. Indeed, in the nonrelativistic framework
one employs the free space relation to relate the lower to the upper
component of the Dirac spinor instead of determining the lower component
dynamically through the Dirac equation. Hence, any evidence of possible
medium modifications to the ratio of lower-to-upper components of the
Dirac spinors is lost.
 
	
Using the QHD theory developed above one finds that there are three
non-vanishing ground state densities for spherical and spin-saturated
nuclei. These are the conventional matter (vector) density defined by
%%%
\begin{equation}
  \rho_{\lower 3pt \hbox{$\scriptstyle V$}}(r) = \sum_{\alpha}^{\rm
  occ} \overline{{\cal U}}_{\alpha}({\bf x})\,
  \gamma^{{\scriptscriptstyle 0}} \, {\cal U}_{\alpha}({\bf x}) \,,
  \quad
\end{equation}
which leads to the vector density given by
\begin{equation}
   \rho_{\lower 3pt \hbox{$\scriptstyle V$}}(r) = \sum_{a}^{\rm occ}
   \left({2j_{a}+1 \over 4\pi r^{2}}\right) \Big(g_{a}^2(r) +
   f_{a}^2(r)\Big) \,,
\label{rhov}
\end{equation}
%%%
where ${\cal U}_{\alpha}({\bf x})$ is a single-particle Dirac spinor
(solution to Dirac equation) for the bound nucleon, $g_{a}(r)$ and
$f_{a}(r)$ are the radial parts of the upper and lower components of
the Dirac spinor, respectively, and the above sums run over all the
occupied single-particle states in the nucleus. Analogously, the
scalar density is defined by
%%%
\begin{equation}
  \rho_{\lower 3pt \hbox{$\scriptstyle S$}}(r) = \sum_{\alpha}^{\rm
  occ} \overline{{\cal U}}_{\alpha}({\bf x})\, {\cal U}_{\alpha}({\bf
  x}) \,, \quad
\end{equation}
leading to it given as
\begin{equation}
   \rho_{\lower 3pt \hbox{$\scriptstyle S$}}(r) = \sum_{a}^{\rm occ}
   \left({2j_{a}+1 \over 4\pi r^{2}}\right) \Big(g_{a}^2(r) -
   f_{a}^2(r)\Big) \,.
\label{rhos}
\end{equation}
%%%
Finally, we have the tensor density defined by
%%%
\begin{equation}
  \Big[ \rho_{\lower 3pt \hbox{$\scriptstyle T$}}(r)\,\hat{r}
    \Big]^{i} = \sum_{\alpha}^{\rm occ} \overline{{\cal
    U}}_{\alpha}({\bf x})\, \sigma^{{\scriptscriptstyle 0}i} \, {\cal
    U}_{\alpha}({\bf x}) \,, \quad
\end{equation}
resulting in the following expression for $\rho_{\lower 3pt
\hbox{$\scriptstyle T$}}(r)$
\begin{equation}
   \rho_{\lower 3pt \hbox{$\scriptstyle T$}}(r) = \sum_{a}^{\rm occ}
   \left({2j_{a}+1 \over 4\pi r^{2}}\right) 2g_{a}(r)f_{a}(r) \,.
   \label{rhotr}
\end{equation}
%%%
The axial-vector density as well as the pseudoscalar density can be
defined in analogous fashion to these three non-vanishing densities. In Chapter \ref{ch:CoherentTheory} the consequences of having
three fundamentally different and non-vanishing densities and their role in the
photoproduction process will be clarified.

\section{An Example of a Relativistic Nuclear Structure Calculation: ${}^{40}$Ca}


In this section, I will discuss a specific example of a nuclear
structure calculation to present you with a manifestation of using
this formalism. Figure \ref{fig:protonElevelsCa40} illustrates a
comparison between our calculations and the experimental data for the
proton level diagram of ${}^{40}$Ca.
%%%
\BFIG
\centerline{\psfig{figure=Ca40EneLevel.pstex,height=6.0in,width=4.50in}}
\caption[Energy level diagram for ${}^{40}$Ca]
{A comparison between our calculations (QHD-II) and the experimental data
for the proton level diagram of ${}^{40}$Ca. The experimental measurements are obtained from ($p, 2p$)~\cite{ray79} and ($e,
e^{\prime} p$)~\cite{naket76,mouet76} experiments.}
\label{fig:protonElevelsCa40}
\EFIG
%%% 
The experimental measurements are obtained from ($p, 2p$)~\cite{ray79} and ($e,
e^{\prime} p$)~\cite{naket76,mouet76} experiments. The theoretical calculations for this figure are done using the QHD-II
model. As can be seen, this model predicts properly the shell
structure of ${}^{40}$Ca with the accurate level ordering and spacing
as well as the proper magnitude for the spin-orbit splitting.


Figure \ref{fig:protonQHD-IvsQHD-II} shows the proton spectrum
calculated using QHD-I and QHD-II models.
%%%
\BFIG
\centerline{\psfig{figure=pQHD-IvsQHD-II.pstex,height=6.0in,width=4.5in}}
\caption[Comparison between QHD-I and QHD-II results for the
proton spectrum in ${}^{40}$Ca] {A comparison between QHD-I and QHD-II
results for the proton spectrum in ${}^{40}$Ca. The QHD-II results are
shifted positively in energy due to the Coulomb repulsion.}
\label{fig:protonQHD-IvsQHD-II}
\EFIG
%%% 
It is evident that apart from an overall positive shift of the
energies in the QHD-II model calculations, the two level diagrams are
essentially identical. This shift is a realization of including the
Coulomb repulsion in the QHD-II model.  Figure
\ref{fig:neutronQHD-IvsQHD-II} displays the same comparison but this
time for the neutron spectrum.
%%%
\BFIG
\centerline{\psfig{figure=nQHD-IvsQHD-II.pstex,height=6.0in,width=4.50in}}
\caption[Comparison between QHD-I and QHD-II results for the
neutron spectrum in ${}^{40}$Ca] {A comparison between QHD-I and
QHD-II results for the neutron spectrum in ${}^{40}$Ca. Since neutrons
are not affected by the Coulomb repulsion, the two results are
essentially identical.}
\label{fig:neutronQHD-IvsQHD-II}
\EFIG
%%% 
Since neutrons do not feel the Coulomb repulsion, the spectrum using
QHD-II is identical to that using QHD-I apart from minute differences.
The differences arise from the inclusion of the $\rho$ meson which
couples differently to the protons and neutrons as well as from
indirect nonlinear effects originating from the Coulomb repulsion in
the proton sector.

Figure \ref{fig:Ca40desities} exhibits various nuclear densities for
${}^{40}$Ca determined using the QHD-II model.
%%%
\BFIG
\centerline{\psfig{figure=Ca40densities.pstex,height=5.5in,width=6.0in}}
\caption[Various nuclear densities in ${}^{40}$Ca]
{Various nuclear densities in ${}^{40}$Ca: the vector (matter) density
$\rho_v$, the scalar density $\rho_s$, the iso-vector density
$\rho_{iso}$ (the difference between the proton and the neutron vector
densities in the nucleus), and the charge density $\rho_{ch}$.}
\label{fig:Ca40desities}
\EFIG
%%% 
It includes the vector (matter) density $\rho_v$, the scalar density
$\rho_s$, the iso-vector density $\rho_{iso}$ (the difference between
the proton and the neutron vector densities in the nucleus), and the
charge density $\rho_{ch}$. These densities generate the four
different potentials in the nucleus: the $\sigma$ scalar potential
$g_s \phi(r)$, the $\omega$ vector potential $g_v V(r)$, the $\rho$ vector
potential $\frac{1}{2} g_\rho {b(r)}$, and the photon (electromagnetic) vector
potential $e A(r)$ respectively. These potentials are shown in Figure
\ref{fig:Ca40potentials}.
%%%
\BFIG
\centerline{\psfig{figure=Ca40potential.pstex,height=5.5in,width=6.0in}}
\caption[The different potentials in ${}^{40}$Ca]
{The different potentials in ${}^{40}$Ca: the $\sigma$ scalar
potential $g_s\phi(r)$, the $\omega$ vector potential $g_v V(r)$, the
$\rho$ vector potential $\frac{1}{2} g_\rho b(r)$, and the photon (electromagnetic)
vector potential $e A(r)$. The $b(r)$ and $A(r)$ potentials have been
magnified by a factor of ten for better display.}
\label{fig:Ca40potentials}
\EFIG
%%% 
In this figure, the $b(r)$ and $A(r)$ potentials have been magnified
by a factor of ten for a better display.




